Towards Compositional Adversarial Robustness: Generalizing Adversarial Training to Composite Semantic Perturbations

Model robustness against adversarial examples of single perturbation type such as the $\ell_{p}$-norm has been widely studied, yet its generalization to more realistic scenarios involving multiple semantic perturbations and their composition remains largely unexplored. In this paper, we first propose a novel method for generating composite adversarial examples. Our method can find the optimal attack composition by utilizing component-wise projected gradient descent and automatic attack-order scheduling. We then propose generalized adversarial training (GAT) to extend model robustness from $\ell_{p}$-ball to composite semantic perturbations, such as the combination of Hue, Saturation, Brightness, Contrast, and Rotation. Results obtained using ImageNet and CIFAR-10 datasets indicate that GAT can be robust not only to all the tested types of a single attack, but also to any combination of such attacks. GAT also outperforms baseline $\ell_{\infty}$-norm bounded adversarial training approaches by a significant margin.

==> preprint/assets/figs/loss_landscape/loss_models.tex <==
\begin{figure*}[htbp]
     \centering
     \includegraphics[width=1\linewidth, trim=0.1cm 0.1cm 0.1cm 0.1cm, clip]{preprint/assets/figs/loss_landscape/loss-landscape-between-models.pdf}
     \caption{The loss landscapes of each single semantic attack with different WideResNet34 training models.}
     \label{fig:appendix_models_loss}
\end{figure*}


==> preprint/assets/tables/attack_power.tex <==
\begin{table*}[ht]
  \centering
    \begin{tabular}{l|c|c|c|c|c|c}
    \toprule
        & Hue, $\epsilon_h$ &  Saturate, $\epsilon_s$ &  Bright, $\epsilon_b$ & Contrast, $\epsilon_c$ &  Rotate, $\epsilon_\theta$ & $\ell_{\infty}$, $\epsilon_{\ell}$   \\
    \midrule
    CIFAR-10 & $-\pi \sim \pi$ & $0.7 \sim 1.3$ & $-0.2 \sim 0.2$ & $0.7 \sim 1.3$ & $-10\degree \sim 10\degree$ & 8/255 \\
    \midrule
    ImageNet & $-\pi \sim \pi$ & $0.7 \sim 1.3$ & $-0.2 \sim 0.2$ & $0.7 \sim 1.3$ & $-10\degree \sim 10\degree$ & 4/255 \\
    \bottomrule
    \end{tabular}%
  \caption{}%
  \label{tab:attack_epsilon_setting}%
\end{table*}%

==> preprint/assets/tables/cifar10_3attack_ra.tex <==
\begin{table}[t]
\setlength\tabcolsep{8pt}
  \centering
   \caption{Comparison of robust accuracy (\%) against 3 composite adversarial attacks (\textit{CAA}$_{3}$) with scheduled ordering, including 3 combinations: \textit{CAA}$_{3a}$: (Hue, Saturation, $\ell_{\infty}$), \textit{CAA}$_{3b}$: (Hue, Rotation, 
  $\ell_{\infty}$), \textit{CAA}$_{3c}$: (Brightness, Contrast, $\ell_{\infty}$), on CIFAR-10}%
  \label{tab:three_ra}%
    \begin{tabular}{l|r|rrr} 
    \toprule
    Training  & Clean & \textit{CAA}$_{3a}$  &  \textit{CAA}$_{3b}$  &  \textit{CAA}$_{3c}$  \\
    \midrule
    Normal$^\dagger$ & 95.3  & 0.0 & 0.0 & 0.0 \\
    Madry$_{\infty}^{\dagger}$ & 87.0  & 30.8 & 19.1 & 19.7 \\
    PAT$_{self}^\dagger$ & 82.4  & 21.1 & 12.5 & 18.4 \\
    PAT$_{alex}^\dagger$ & 71.6  & 21.1 & 12.5 & 17.2 \\
    \textbf{GAT-f}$^\dagger$ & 86.5  & 36.3 & 29.3 & 25.6 \\
     \textbf{GAT-fs}$^\dagger$ & 82.6 & \textbf{42.1} & \textbf{35.4} & \textbf{30.7} \\
    \midrule
    Normal$^\ast$ & 94.0  & 0.0 & 0.0 & 0.0 \\
    Trades$_{\infty}^\ast$ & 84.9  & 30.1 & 20.8 & 10.5 \\
    FAT$_{\infty}^\ast$ & 88.1  & 30.4  & 17.4  & 13.2 \\
    AWP$_{\infty}^\ast$ & 85.4  & 34.6  & 23.6  & 11.8 \\
    \textbf{GAT-f}$^\ast$ & 85.4  & 43.6 & \textbf{37.8} & 32.3 \\
     \textbf{GAT-fs}$^\ast$ & 83.2  & \textbf{43.8} & \textbf{37.8} & \textbf{33.4} \\
    \bottomrule
    \end{tabular}%
 \vspace{-4mm}
\end{table}%


==> preprint/assets/tables/cifar10_computation_cost.tex <==
\vspace{-3mm}\begin{table}[h]
    \centering
\setlength\tabcolsep{3pt}
\adjustbox{max width=0.85\linewidth}{%
    \centering
    \begin{tabular}{rrrrrrr|rr}
    \toprule
    \multicolumn{1}{l}{Hue} & \multicolumn{1}{l}{Sat.} & \multicolumn{1}{l}{Rot.} & \multicolumn{1}{l}{Bri.} & \multicolumn{1}{l}{Cont.} & \multicolumn{1}{l}{PGD} & \multicolumn{1}{l|}{Auto-Attack} & \multicolumn{1}{l}{Semantic} & \multicolumn{1}{l}{Full} \\
    \midrule
    0.8s  & 0.8s  & 0.8s  & 0.7s  & 0.8s  & 0.7s & 261s & 81s & 102s \\
    \bottomrule
    \end{tabular}}%
    \vspace{-3mm}
    \caption{Comparison of computing time of one/multiple attacks.}
    \label{tab:computation_time}
\end{table}
\vspace{-4mm}

==> preprint/assets/tables/cifar10_ra.tex <==
% Table generated by Excel2LaTeX from sheet 'single'
\begin{table}[t]
\setlength\tabcolsep{5.9pt}
\centering
    \caption{Comparison of accuracy (\%)  on CIFAR-10. %The notation $\dagger$ means the model architecture is ResNet50 and $\ast$ is WideResNet34
    }
    \label{tab:cifar10_ra}%
    \begin{tabular}[table-number-alignment = center]{l|r|rr|rr}
    \toprule
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &        \multicolumn{2}{c|}{Semantic attacks}  & \multicolumn{2}{c}{Full attacks}\\
    Training  & Clean & Rand. & Sched. & Rand. & Sched. \\
    \midrule
    Normal$^\dagger$ & 95.3  & 59.6  & 44.8  & 0.0  & 0.0  \\
    Madry$_{\infty}^{\dagger}$ & 87.0  & 31.3  & 21.6  & 10.9  & 3.9 \\
    PAT$_{self}^\dagger$ & 82.4  & 28.6  & 18.0  & 9.3  & 3.0  \\
    PAT$_{alex}^\dagger$ & 71.6  & 23.4  & 12.9  & 10.2  & 2.8  \\
    %\textbf{GAT-s}$^\dagger$ & 80.9  & 18.1  & 6.8  & 0.0  & 0.0  \\
    \textbf{GAT-f}$^\dagger$ & 86.5  & \textbf{76.0} & \textbf{72.7} & 26.3 & 15.8 \\
     \textbf{GAT-fs}$^\dagger$ & 82.6 &  71.1 & 67.7 & \textbf{31.8} & \textbf{21.5} \\
    \midrule
    Normal$^\ast$ & 94.0  & 45.6  & 30.6  & 0.0  & 0.0  \\
    Trades$_{\infty}^\ast$ & 84.9  & 16.4  & 8.7  & 5.8  & 1.8  \\
    FAT$_{\infty}^\ast$ & 88.1  & 18.5  & 10.5  & 6.3  & 1.7  \\
    AWP$_{\infty}^\ast$ & 85.4  & 15.4  & 8.0  & 6.0  & 1.8  \\
    %\textbf{GAT-s}$^\ast$ & 91.0  & 33.8  & 19.1  & 0.0  & 0.0  \\
    \textbf{GAT-f}$^\ast$ & 85.4  & \textbf{73.8} & \textbf{70.3} & 31.9 & 21.7 \\
     \textbf{GAT-fs}$^\ast$ & 83.2  &  71.0  & 67.2  & \textbf{33.1}  & \textbf{22.8} \\
    \bottomrule
    \end{tabular}
    \vspace{-4mm}
    % Additional detail of baseline models are described in Appendix~\ref{subsec:model_detail}
    %We report the robust accuracy (\%) on test sets generated by the method proposed in Sec.~\ref{sec:method}. 
    %The results are summarized in SubSec.~\ref{subsec:exp} and the additional detail of baseline models are described in Appendix}%
\end{table} 


==> preprint/assets/tables/cifar10_traditional_attacks.tex <==
\vspace{-3mm}
\begin{table}[h]
\setlength\tabcolsep{9pt}
\def\arraystretch{0.85}%
    \centering
\adjustbox{max width=\linewidth}{%
    \centering
    \begin{tabular}{l|r|rrrr|rr}
    \toprule
     & & \multicolumn{4}{c|}{Traditional attacks ($\ell_\infty$)} & \multicolumn{2}{c}{Full attacks}\\
     Training & Clean & PGD & FGSM & BIM & FAB & Rand. & Sched. \\
     \midrule
    Normal$^\dagger$ & 95.2  & 0.0  & 24.5  & 0.0   & 0.2   & 0.0   & 0.0 \\
    Madry$_{\infty}^{\dagger}$ & 87.0  & 53.5  & 61.4  & 53.8  & 52.6  & 10.8  & 3.7 \\
    PAT$_{self}^\dagger$ & 82.4  & 41.2  & 54.6  & 42.1  & 43.3  & 9.1   & 2.5 \\
    PAT$_{alex}^\dagger$ & 71.6  & 41.9  & 50.2  & 45.0  & 40.6  & 10.3  & 2.5 \\
    \textbf{GAT-f}$^\dagger$ & 82.3  & 42.7  & 52.2  & 43.0  & 43.1  & 30.0    & 18.8 \\
    \textbf{GAT-fs}$^\dagger$ & 82.1  & 46.6  & 55.0  & 47.1  & 45.9  & 32.3  & 21.8 \\
    \bottomrule
    \end{tabular}}%
    \vspace{-3mm}
    \caption{Comparison of accuracy (\%) on CIFAR-10 (ResNet-50).}
    \label{tab:traditional_attacks}
\end{table}
\vspace{-3mm}

==> preprint/assets/tables/imagenet/two_ra.tex <==
% Table generated by Excel2LaTeX from sheet 'single'
\begin{table*}[ht]
  \centering
    \begin{tabular}{l|r|rrrrr} 
    \toprule
    \multicolumn{1}{c|}{}  &       & \multicolumn{5}{c}{2 attacks ($\ell_{\infty}$ + \textit{one of semantic attacks})} \\
    Training & \multicolumn{1}{c|}{Clean} & Hue & Saturate & Rotation & Brightness & Contrast \\
    \midrule
    Normal$^\dagger$ & 76.1  & 0.1 (76.1) & 0.1 (76.1) & 0.1 (76.1) & 0.1 (76.1) & 0.1 (76.1) \\
    Madry$_{\infty}^{\dagger}$ & 62.4  & 20.8 (41.6) & 31.1 (31.3) & 27.3 (35.1) & 28.9 (33.6) & 29.4 (33.1) \\
    Fast-AT$^\dagger$ & 53.8  & 14.8 (39) & 24.4 (29.4) & 19.9 (34) & 21.4 (32.4) & 22 (31.8) \\
    \textbf{GAT-f}$^\dagger$ & 60.0  & 22.6 (37.4) & 25.2 (34.7) & 25.3 (34.6) & 25.4 (34.5) & 24.1 (35.9) \\
    \bottomrule
    \end{tabular}%
  \caption{Robust accuracy of two attacks.}%
  \label{tab:appendix_imagenet_two_ra}%
\end{table*}%


==> preprint/assets/tables/imagenet_3attack_ra.tex <==
\begin{table}[t]
  \setlength\tabcolsep{8pt}
  \centering
  \caption{Comparison of robust accuracy (\%) against \textit{CAA}$_{3a}$, \textit{CAA}$_{3b}$, and \textit{CAA}$_{3c}$ on ImageNet (same combination as Table \ref{tab:three_ra})}%
  \label{tab:imagenet_three_ra}%
    \begin{tabular}{l|r|rrr} 
    \toprule
    Training  & Clean & \textit{CAA}$_{3a}$  &  \textit{CAA}$_{3b}$  &  \textit{CAA}$_{3c}$  \\
    \midrule
    Normal$^\dagger$ & 76.1  & 0.0 & 0.0 & 0.0 \\
    Madry$_{\infty}^{\dagger}$ & 62.4  & 14.5 & 9.6 & 17.4 \\
    Fast-AT$^\dagger$ & 53.8  & 9.9 & 5.4 & 10.2 \\
    \textbf{GAT-f}$^\dagger$ & 60.0  & \textbf{17.7} & \textbf{16.9} & \textbf{19.1} \\
    \bottomrule
    \end{tabular}%
    \vspace{-4mm}
\end{table}%


==> preprint/assets/tables/imagenet_ra.tex <==
% Table generated by Excel2LaTeX from sheet 'single'
\begin{table}[t]
\setlength\tabcolsep{5.85pt}
\centering
    \caption{Comparison of accuracy (\%) on ImageNet}
    \label{tab:imagenet_ra}%
    \begin{tabular}[table-number-alignment = center]{l|r|rr|rr}
    \toprule
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &        \multicolumn{2}{c|}{Semantic attacks}  & \multicolumn{2}{c}{Full attacks}\\
    Training  & Clean & Rand. & Sched. & Rand. & Sched. \\
    \midrule
    Normal$^\dagger$ & 76.1  & 30.7  & 19.1  & 0.0  & 0.0  \\
    Madry$_{\infty}^{\dagger}$ & 62.4  & 14.1  & 9.0  & 7.1  & 3.1  \\
    Fast-AT$^\dagger$ & 53.8  & 6.2  & 3.5  & 3.3  & 1.2  \\
    \textbf{GAT-f}$^\dagger$ & 60.0  & \textbf{40.7} & \textbf{36.2} & \textbf{17.8} & \textbf{11.7} \\
    \bottomrule
    \end{tabular}
    \vspace{-4mm}
\end{table} 

